RMGS-SLAM: Real-time Multi-sensor Gaussian Splatting SLAM

Achieving real-time Simultaneous Localization and Mapping (SLAM) based on 3D Gaussian splatting (3DGS) in large-scale real-world environments remains challenging, as existing methods still struggle to jointly achieve low-latency pose estimation, continuous 3D Gaussian reconstruction, and long-term global consistency. In this paper, we present a tightly coupled LiDAR-Inertial-Visual 3DGS-based SLAM framework for real-time pose estimation and photorealistic mapping in large-scale real-world scenes. The system executes state estimation and 3D Gaussian primitive initialization in parallel with global Gaussian optimization, enabling continuous dense mapping. To improve Gaussian initialization quality and accelerate optimization convergence, we introduce a cascaded strategy that combines feed-forward predictions with geometric priors derived from voxel-based principal component analysis. To enhance global consistency, we perform loop closure directly on the optimized global Gaussian map by estimating loop constraints through Gaussian-based Generalized Iterative Closest Point registration, followed by pose-graph optimization. We also collect challenging large-scale looped outdoor sequences with hardware-synchronized LiDAR-camera-IMU and ground-truth trajectories for realistic evaluation. Extensive experiments on both public datasets and our dataset demonstrate that the proposed method achieves a state of the art among real-time efficiency, localization accuracy, and rendering quality across diverse real-world scenes.

==> Figures_tex/gaussian_init.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{Figures/gaussian_init.pdf}
    \caption{Cascaded 3D Gaussian Primitives Initialization.
    The initialization follows a cascaded strategy that progressively integrates feed-forward predictions with voxel-PCA-based geometric priors to improve both structural consistency and optimization convergence.}
    \label{fig:cascaded_init}
\end{figure}

% \footnotetext{Feed-forward predictions provide anisotropic shape priors, while voxel-PCA supplies geometry-aware orientation and scale estimation when reliable; otherwise, isotropic fallback is adopted.}

==> Figures_tex/sh_difference.tex <==
% Usage:
%   \input{tex/qualitative_grid_6cols_last2rows}
% Required package in main preamble:
%   \usepackage{graphicx}

\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{1.0}
\providecommand{\imgw}{0.160\textwidth}
\providecommand{\qimg}[1]{\includegraphics[width=\imgw]{#1}}

\begin{tabular}{cccccc}
\textbf{GS-LIC2} & \textbf{GS-LIVM} & \textbf{MonoGS} & \textbf{SplaTAM} & \textbf{Ours} & \textbf{GT} \\
\qimg{Figures/render_figures_inset/scene03_lecture_01/05_gslic2/scene03_lecture_01_05_gslic2_img01_inset.jpg} &
\qimg{Figures/render_figures_inset/scene03_lecture_01/04_gslivm/scene03_lecture_01_04_gslivm_img01_inset.png} &
\qimg{Figures/render_figures_inset/scene03_lecture_01/02_monogs/scene03_lecture_01_02_monogs_img01_inset.png} &
\qimg{Figures/render_figures_inset/scene03_lecture_01/03_splatam/scene03_lecture_01_03_splatam_img01_inset.png} &
\qimg{Figures/render_figures_inset/scene03_lecture_01/01_ours/scene03_lecture_01_01_ours_img01_inset.png} &
\qimg{Figures/render_figures_inset/scene03_lecture_01/00_ground_truth/scene03_lecture_01_00_ground_truth_img01_inset.png} \\

\qimg{Figures/render_figures_inset/scene03_lecture_01/05_gslic2/scene03_lecture_01_05_gslic2_img02_inset.jpg} &
\qimg{Figures/render_figures_inset/scene03_lecture_01/04_gslivm/scene03_lecture_01_04_gslivm_img02_inset.png} &
\qimg{Figures/render_figures_inset/scene03_lecture_01/02_monogs/scene03_lecture_01_02_monogs_img02_inset.png} &
\qimg{Figures/render_figures_inset/scene03_lecture_01/03_splatam/scene03_lecture_01_03_splatam_img02_inset.png} &
\qimg{Figures/render_figures_inset/scene03_lecture_01/01_ours/scene03_lecture_01_01_ours_img02_inset.png} &
\qimg{Figures/render_figures_inset/scene03_lecture_01/00_ground_truth/scene03_lecture_01_00_ground_truth_img02_inset.png} \\
\end{tabular}

\caption{Qualitative comparison of rendering results on two selected frames from the \textit{Lecture\_01} sequence. Both frames depict the same local region under different viewpoints and lighting conditions. From left to right, the columns correspond to GS-LIC2, GS-LIVM, MonoGS, SplaTAM, our method, and ground truth (GT). The comparison reflects the different abilities of the methods to capture view-dependent appearance changes, which are largely affected by the spherical harmonics (SH) degree of the Gaussian representation.}
\label{fig:sh_difference}
\end{figure*}


==> Tables_tex/1_render_estimate.tex <==
\begin{table*}[!t]
\centering
\caption{Rendering quality comparison on all datasets.}
\label{tab:rendering_results}
\footnotesize
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{5.5pt}
%\resizebox{\textwidth}{!}{
\begin{tabular}{ll*{12}{C{1.08cm}}}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Metric} & \multicolumn{12}{c}{Datasets} \\
\cmidrule(l){3-14}
&
& \shortstack{HKairport\\03}
& \shortstack{HKisland\\03}
& \shortstack{CBD\\Building02}
& \shortstack{HKU\\Campus}
% & \shortstack{HKU\\Landmark}
& \shortstack{Lecture\\Center01}
& \shortstack{Retail\\Street}
& \shortstack{SCU\\01}
& \shortstack{SCU\\02}
& \shortstack{NUS\\01}
% & \shortstack{NUS\\02}
& Average \\
\midrule
\multirow{3}{*}{Gaussian-LIC2}
& PSNR$\uparrow$
& 14.55 % 14.547
& 17.65 % 17.651
& 22.30 % 22.295
& 27.08 % 27.080
& 31.28 % 31.278
& 24.37
& \textbf{23.72} % 25.171
& $\times$
& 23.01 % 23.010
& 23.18 \\

& SSIM$\uparrow$
& 0.38 % 0.375
& 0.44 % 0.440
& 0.73 % 0.729
& 0.76 % 0.761
& 0.91 % 0.911
& 0.78 % 0.776
& \textbf{0.81} % 0.847
& $\times$
& \textbf{0.84} % 0.835
& 0.71 \\ % 0.712

& LPIPS$\downarrow$
& 0.62 % 0.621
& 0.57 % 0.566
& 0.31 % 0.306
& 0.20 % 0.203
& 0.18 % 0.178
& 0.12
& \textbf{0.23} % 0.183
& $\times$
& \textbf{0.22} % 0.224
& 0.30 \\ % 0.301
\cdashline{1-14}

\multirow{3}{*}{GS-LIVM}
& PSNR$\uparrow$
& $\times$
& $\times$
& 9.87 % 9.870
& 17.77 % 17.765
& 21.72 % 21.720
& 10.16 % 10.156
& 16.22 % 16.215
& 15.09 % 15.091
& 15.95 % 15.945
& 15.25 \\ % 15.251

& SSIM$\uparrow$
& $\times$
& $\times$
& 0.46 % 0.463
& 0.53 % 0.532
& 0.78 % 0.780
& 0.42 % 0.421
& 0.54 % 0.543
& 0.55 % 0.549
& 0.60 % 0.603
& 0.55 \\ % 0.556

& LPIPS$\downarrow$
& $\times$
& $\times$
& 0.80 % 0.796
& 0.64 % 0.638
& 0.53 % 0.527
& 0.82 % 0.818
& 0.44 % 0.444
& 0.52 % 0.518
& 0.61 % 0.607
& 0.62 \\ % 0.621
\cdashline{1-14}

\multirow{3}{*}{MonoGS}
& PSNR$\uparrow$
& 15.93 % 15.930
& $\times$
& 21.76 % 21.755
& \textbf{30.36} % 30.360
& 29.81 % 29.805
& 22.81 % 22.806
& 22.41 % 22.408
& \textbf{23.01} % 23.007
& \textbf{23.33} % 23.327
& \textbf{23.68} \\ % 23.678

& SSIM$\uparrow$
& 0.37 % 0.368
& $\times$
& 0.72 % 0.715
& 0.84 % 0.841
& 0.90 % 0.904
& 0.71 % 0.714
& 0.73 % 0.729
& \textbf{0.75} % 0.754
& 0.82 % 0.819
& 0.73 \\ % 0.731

& LPIPS$\downarrow$
& 0.58 % 0.576
& $\times$
& 0.30 % 0.302
& 0.21 % 0.212
& 0.25 % 0.247
& 0.27 % 0.271
& 0.45 % 0.448
& 0.36 % 0.362
& 0.27 % 0.274
& 0.34 \\ % 0.337
\cdashline{1-14}

\multirow{3}{*}{Ours}
& PSNR$\uparrow$
& \textbf{20.11} % 20.1151 % previous 19.444
& \textbf{19.44} % 19.441
& \textbf{26.20} % 26.196
& 28.48 % 28.482
& \textbf{34.40} % 34.396
& \textbf{26.89} % 26.8931 % previous 24.568
& 20.61 % 20.612
& 20.07 % 20.067
& 19.41 % 19.411
& 23.62 \\ % 23.624

& SSIM$\uparrow$
& \textbf{0.56} % 0.556816 % previous 0.588
& \textbf{0.59} % 0.588
& \textbf{0.91} % 0.906
& \textbf{0.85} % 0.853
& \textbf{0.95} % 0.949
& \textbf{0.89} % 0.888096 % previous 0.765
& 0.77 % 0.767
& 0.72 % 0.718
& 0.74 % 0.744
& \textbf{0.77} \\ % 0.764

& LPIPS$\downarrow$
& \textbf{0.32} % 0.318059 % previous 0.431
& \textbf{0.45} % 0.450
& \textbf{0.12} % 0.120
& \textbf{0.15} % 0.154
& \textbf{0.12} % 0.119
& \textbf{0.09} % 0.094294 % previous 0.174
& 0.29 % 0.294
& \textbf{0.31} % 0.312
& 0.38 % 0.380
& \textbf{0.27} \\ % 0.270
\bottomrule
\end{tabular}

\vspace{0.8mm}
\begin{minipage}{\textwidth}
\raggedright
\scriptsize
\textit{Note:} Higher PSNR and SSIM indicate better rendering quality, whereas lower LPIPS indicates better perceptual similarity. $\times$ denotes that the dataset and method was unable to finish running on our experimental setup.
\end{minipage}
\end{table*}

==> Tables_tex/2_pose_estimate.tex <==
\begin{table*}[t]
\centering
\caption{Pose accuracy comparison on different datasets.}
\label{tab:pose_results}
\footnotesize
% \small
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{11.8pt}
%\resizebox{\textwidth}{!}
% \begin{tabular}{lcccccccccccc}
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{Method}
& \multicolumn{2}{c}{HKairport03}
& \multicolumn{2}{c}{HKisland03}
& \multicolumn{2}{c}{SCU\_01}
& \multicolumn{2}{c}{SCU\_02}
& \multicolumn{2}{c}{NUS\_01} \\ 
% & \multicolumn{2}{c}{NUS\_02} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} %\cmidrule(lr){12-13}
& ATE$\downarrow$ & RPE$\downarrow$
& ATE$\downarrow$ & RPE$\downarrow$
& ATE$\downarrow$ & RPE$\downarrow$
& ATE$\downarrow$ & RPE$\downarrow$
& ATE$\downarrow$ & RPE$\downarrow$ \\
% & ATE$\downarrow$ & RPE$\downarrow$ \\
\midrule
FAST-LIVO2~\cite{zheng2024fast}
& 1.44 % 1.439
& 2.22 % 2.219
& 2.63 % 2.629
& \textbf{2.03} % 2.033
& 2.74 % 2.735
& 0.49 % 0.494
& 3.60 % 3.596
& 0.40 % 0.397
& 1.02 % 1.016
& 0.04 \\ % 0.037
% & 0.125 & 0.038 \\
R3LIVE~\cite{lin2022r}
& 130.12 % 130.123
& 3.96 % 3.960
& 96.15 % 96.153
& 2.35 % 2.351
& 35.00 % 35.001
& 0.46 % 0.460
& 0.88 % 0.882
& 0.41 % 0.412
& \textbf{0.22} % 0.215
& 0.04 \\ % 0.0384
% & 0.125 & 0.038 \\
Gaussian-LIC2~\cite{lang2025gaussian2_gaussian_lic2}
& $\times$ %28.89 % 28.891
& $\times$ %2.50 % 2.499
& $\times$ %20.90 % 20.904
& $\times$ %2.62 % 2.624
& 2.70 % 2.763
& \textbf{0.09} % 0.086
& $\times$ & $\times$
& 1.04 % 1.045
& \textbf{0.01} \\ % 0.006
% & 0.125 & 0.038 \\
GS-LIVM~\cite{xie2025gs}
& $\times$ & $\times$
& $\times$ & $\times$
& 3.02 % 3.017
& 0.17 % 0.172
& $\times$ %3.31 % 3.311
& $\times$ %\textbf{0.27} % 0.272
& 1.41 % 1.414
& 0.03 \\ % 0.028
% & 0.125 & 0.038 \\
MonoGS~\cite{matsuki2024gaussian_monoGs}
& 112.72 % 112.716
& \textbf{1.64} % 1.639
& $\times$ & $\times$
& 12.82 % 12.825
& 0.47 % 0.471
& 4.17 % 4.169
& 0.44 % 0.443
& 1.07 % 1.071
& 0.37 \\ % 0.366
% & 0.125 & 0.038 \\
\midrule
Ours
& \textbf{1.36} % 1.356
& 2.22 % 2.216
& \textbf{2.61} % 2.612
& \textbf{2.03} % 2.034
& \textbf{0.93} % 0.933
& 0.94 % 0.938
& \textbf{0.41} % 0.410
& 0.86 % 0.858
& 1.01 % 1.011
& 0.04 \\ % 0.037
% & \textbf{0.102} & \textbf{0.031} \\
\bottomrule
\end{tabular}

\vspace{0.8mm}
\begin{minipage}{\textwidth}
\raggedright
\scriptsize
\textit{Note:} Absolute Trajectory Error (ATE) is reported as RMSE, and Relative Pose Error (RPE) is computed as the mean relative pose error using the \texttt{evo} toolkit. $\times$ denotes that the dataset and method was unable to finish running on our experimental setup.
\end{minipage}
\end{table*}

==> Tables_tex/3_run_time_analysis.tex <==
% \begin{table}[ht]
% \centering
% \caption{Full pipeline runtime comparison on all datasets.}
% \label{tab:e2e_runtime}
% \footnotesize
% \renewcommand{\arraystretch}{1.12}
% \setlength{\tabcolsep}{3pt}
% \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}>{\raggedright\arraybackslash}p{1.7cm}ccccccc@{}}
% \toprule
% Sequence & Bag (s) & G-LIC2 & GS-L & Loop & Mono & MM3D & Ours \\
% \midrule
% HKairport03           & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
% HKisland03            & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
% CBD\_02       & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
% HKU\_Campus            & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
% Landmark          & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
% Lect\_Center01  & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
% Retail\_Street         & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
% SCU 01                & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
% SCU 02                & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
% NUS 01                & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
% NUS 02                & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
% \midrule
% Avg.                  & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
% \bottomrule
% \end{tabular*}

% \vspace{0.6mm}
% \begin{minipage}{\columnwidth}
% \raggedright
% \scriptsize
% \textit{Note:} Bag denotes the rosbag duration measured from the first to the last ROS timestamp. Runtime denotes the wall-clock time required to process the entire bag.
% \end{minipage}
% \end{table}


\begin{table*}[ht]
\centering
\caption{Full pipeline runtime comparison on all datasets.}
\label{tab:e2e_runtime}
\footnotesize
\renewcommand{\arraystretch}{1.12}
\setlength{\tabcolsep}{2.6pt}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}>{\raggedright\arraybackslash}p{1.8cm}
c
cc cc cc cc cc@{}}
\toprule
\multirow{2}{*}{Sequence}
& \multirow{2}{*}{Full Bag}
& \multicolumn{2}{c}{G-LIC2}
& \multicolumn{2}{c}{GS-LIVM}
& \multicolumn{2}{c}{Loop}
& \multicolumn{2}{c}{Mono}
& \multicolumn{2}{c}{Ours} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
&
& Alg. & Bag
& Alg. & Bag
& Alg. & Bag
& Alg. & Bag
& Alg. & Bag \\
\midrule
HKairport03    & 241.7& 380.4 & 53, 0.3x & $\times$ & $\times$ & 4499.7 & 241.7 & 2044.5 & 66.1 & 385.1 & 241.7, 1x \\
HKisland03     & 235.9 & 283.9& 74.3, 0.5x & $\times$ & $\times$ & 733.3 & 116.5 & $\times$ & $\times$ & 338.2 & 235.9, 1x \\
CBD\_02        & 233.9 & 313.9 & 233.9, 0.8x & 261.9 & 233.9, 1x & 1902.2 & 130.9 & 800.6 & 130.5 & 237.6 & 233.9, 1x \\
HKU\_Campus & 91 & 138.4 & 91, 0.7x & 93.9 & 91, 1x & 1270.8 & 91 & 580.6 & 91 & 103.8 & 91, 1x \\
Lect\_Center01 & 77.1 & 85.3 & 77.1, 1x & 78.5 & 77.1, 1x & 996.5 & 77.1 & 500.2 & 77.1 & 79.5 & 77.1, 1x \\
Retail\_Street & 135.5 & 141 & 135.5, 1x & 279.8 & 135.5, 0.5x & 1830.9 & 135.5 & 860.7 & 135.5 & 141 & 135.5, 1x \\
SCU 01         & 324.4 & 882.7 & 324.4, 1x & $\times$ & $\times$ & 4819.9 & 324.4 & 2841.4 & 324.4 & 328.4 & 324.4, 1x \\
SCU 02         & 189.9 & $\times$ & $\times$ & $\times$ & $\times$ & 2786.1 & 189.9 & 1593.2 & 189.9 & 198.5 & 189.9, 1x \\
NUS 01         & 117.3 & 127.1 & 117.3, 1x & 117.3 & 117.3, 1x & 510 & 53.9 & 599.1 & 117.3 & 129 & 117.3, 1x \\
\midrule
Avg.           & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
\bottomrule
\end{tabular*}

\vspace{0.6mm}
\begin{minipage}{\textwidth}
\raggedright
\scriptsize
\textit{Note:} \textit{Full Bag} denotes the full rosbag duration of each sequence. For each method, \textit{Alg.} denotes the runtime of the main online algorithm, and \textit{Bag} denotes the rosbag duration actually used by that method, measured from the first to the last ROS timestamp. $\times$ denotes that the dataset and method was unable to finish running on our experimental setup.
\end{minipage}
\end{table*}

